Incremental Skill Learning of Stable Dynamical Systems

Efficient skill acquisition, representation, and on-line adaptation to different scenarios has become of fundamental importance for assistive robotic applications. In the past decade, dynamical systems (DS) have arisen as a flexible and robust tool to represent learned skills and to generate motion trajectories. This work presents a novel approach to incrementally modify the dynamics of a generic autonomous DS when new demonstrations of a task are provided. A control input is learned from demonstrations to modify the trajectory of the system while preserving the stability properties of the reshaped DS. Learning is performed incrementally through Gaussian process regression, increasing the robot's knowledge of the skill every time a new demonstration is provided. The effectiveness of the proposed approach is demonstrated with experiments on a publicly available dataset of complex motions.

==> Sections/Robot_Experiments.tex <==

\section{Robot Experiments}\label{sec:lwr_experiments}
%\begin{figure*}[!t]
%	\centering
%	\includegraphics[width=\textwidth]{img/Control_Loop.pdf}
%    	\caption{.}
%    	\label{fig:control_loop}
%\end{figure*}
%
%\subsection{Incremental reshaping in Cartesian space}
%\textcolor{red}{Show free-motion and interaction}

%\subsection{Incremental reshaping in joint space}
This experiment shows the scalability of the proposed approach in high dimensional spaces and its ability to reshape high order DS. The task is a point-to-point motion in the joint space from $\bfx_{1}(0) = [35, 55, 15, -65, -15, 50, 90]\tr\,$deg to $\hat{\bfx}_1 = [-60, 30, 30, -70, -15, 85, 15]\tr\,$deg. The original joint position trajectory is obtained by numerically integrating ($\delta t = 0.005\,$s) the second-order DS
\begin{equation}
\label{eq:joint_ds}
	\begin{split}
		\dot{\bfx}_1 &= \bfx_2\\
		\dot{\bfx}_2 &= 2(\hat{\bfx}_1 - \bfx_1) - 2\sqrt{2}\bfx_2
	\end{split}
\end{equation} 
where $\bfx_1 = [\theta_1,\ldots,\theta_7]\tr \in \mathbb{R}^7$ are the joint angles and $\bfx_2 \in \mathbb{R}^7$ the joint velocities. The system (\ref{eq:joint_ds}) has a GAS equilibrium at $\hat{\bfx} = [\hat{\bfx}_1\tr, \mathbf{0}\tr]\tr \in \mathbb{R}^{14}$. The original joint angles trajectories are shown in Fig. \ref{fig:exp_2} (black solid lines).

As shown in Fig. \ref{fig:overview}, following the original trajectory the robot hits an unforeseen obstacle (the red bar). A kinesthetic demonstration is then provided (red lines in Fig. \ref{fig:exp_2}) to avoid the collision. With the reshaped trajectory (blue lines in Fig. \ref{fig:exp_2}) the robot is able to avoid the obstacle (Fig. \ref{fig:overview}) and to reach the desired goal $\hat{\bfx}_1$. Results are obtained with noise variance $\sigma_{n}^{2} = 0.01$, signal variance $\sigma_{k}^{2} = 0.1$, length scale $l=0.02$ and the threshold $\bar{c} = 1\,$rad/s\textsuperscript{2}. With the adopted $\bar{c}$ only $37$ points over $178$ are added to the GP. 

\begin{figure}[!htb]
\centering  
\includegraphics[width=\columnwidth]{img/Ex_joint.pdf}
\caption{Original joint angles trajectories (black lines), the provided demonstration (red lines) and reshaped joint angles trajectories (blue lines) for the joint space collision avoidance experiment.}
\label{fig:exp_2}
\end{figure}
%\begin{itemize}
%	\item \textcolor{red}{Not working because joint do not reach the goal}
%\end{itemize}

%\subsection{Experiments}
%The effectiveness of the proposed approach is demonstrated with two experiments on a KUKA LWR IV+ $7$ DoF manipulator \cite{FRI}. In both experiments, novel demonstrations of the desired position are provided to the robot by kinesthetic teaching. To guarantee a safe physical guidance, the task is interrupted and the robot is putted in the gravity compensation mode\footnote{In this modality, the robot acts as a massless (or very light) object lying in a space without gravity.} as soon as the user touches the robot. The external torques estimation provided by the fast research interface \cite{FRI} is used to detect physical contacts.
%   
%\subsubsection{End-effector Collision Avoidance}
%This experiment shows the ability of the proposed reshaping approach to learn different behaviours in different regions of the space and the possibility to reshape non-linear DS. The task consists in reaching the goal position $\hat{\bfx}_1 = {[}-0.52, 0, 0.02  {]}^{T} m$ with the robot's end-effector while avoiding a box (see Fig. \ref{fig:snap_exp_1}) of size $7\times 7 \times 23 ~cm$. Two boxes are placed in the scene in different positions, one in the region $\mathcal{R}^{+}$ where $y > 0$ (Fig. \ref{fig:snap_exp_1}(a) and \ref{fig:snap_exp_1}(c)), one in the region $\mathcal{R}^{-}$ where $y < 0$ (Fig. \ref{fig:snap_exp_1}(b) and \ref{fig:snap_exp_1}(d)). Hence, the robot has to learn a bi-modal behaviour to avoid collisions in $\mathcal{R}^{+}$ and $\mathcal{R}^{-}$.
%
%The original position trajectory is obtained by numerically integrating ($\delta t = 0.005~s$) the first-order, non-linear DS
%\begin{equation}
%\label{eq:ee_ds}
%		\dot{\bfx}_1 = \bff(\bfx_1-\hat{\bfx}_1)\\
%\end{equation} 
%where $\bfx_1 = [x,y,z]^{T} \in \mathbb{R}^3$ is the end-effector position and $\dot{\bfx}_1 \in \mathbb{R}^3$ is the end-effector linear velocity. The orientation is kept fixed. The original DS (\ref{eq:ee_ds}) is learned from demonstrations by using the SEDS algorithm \cite{SEDS}. The Lyapunov function $V = \frac{1}{2}(\bfx_1-\hat{\bfx}_1)^T(\bfx_1-\hat{\bfx}_1)$ is used to prove that $\hat{\bfx}_1$ is a GAS equilibrium \cite{SEDS}. The original end-effector trajectories are shown in Fig. \ref{fig:exp_1} (black solid lines).
%
%Following the original trajectory generated with initial position $\bfx_{1}(0) = {[}-0.52, 0.5, 0.02 {]}^{T}m$ ($\bfx_{1}(0) = {[}-0.52, -0.5, 0.02 {]}^{T}m$), the robot hits the box (Fig. \ref{fig:snap_exp_1}(a) and \ref{fig:snap_exp_1}(b)). Two demonstrations (one in $\mathcal{R}^{+}$ and one $\mathcal{R}^{-}$) are provided to show to the robot how to avoid the obstacles (brown solid lines in Fig. \ref{fig:exp_1}). The original DS position trajectories (black solid lines in Fig. \ref{fig:exp_1}) are incrementally adapted to follow the demonstrated positions and different avoiding behaviours are effectively learned in $\mathcal{R}^{+}$ and $\mathcal{R}^{-}$. 
%
%The proposed approach locally modifies the DS, in fact demonstrations in $\mathcal{R}^{+}$, being far from $\mathcal{R}^{-}$, do not affect the behaviour in $\mathcal{R}^{-}$ (and vice versa). The equilibrium position $\hat{\bfx}_1 = {[}-0.52, 0, 0.02  {]}^{T} m$ is always reached, empirically proving that the equilibrium is still GAS. Figure \ref{fig:exp_1} also shows the learned behaviours (green in $\mathcal{R}^{+}$ and blue in $\mathcal{R}^{-}$ solid lines) for different initial positions in a 3D view (Fig. \ref{fig:exp_1}(a)) and in the $xz$ plane (Fig. \ref{fig:exp_1}(b) and \ref{fig:exp_1}(c)). In all cases, the robot is able to achieve the task. Snapshots of the learned bi-modal behaviour are depicted in Fig. \ref{fig:snap_exp_1}(c) and \ref{fig:snap_exp_1}(d).  Results are obtained with noise variance $\sigma_{n}^{2} = 0.1$, signal variance $\sigma_{k}^{2} = 1$, length scale $l=0.001$ and the threshold $\bar{c} = 0.04 ~m$. With the adopted $\bar{c}$ only $106$ points over $798$ are added to the GP. 
%
%\begin{figure}
%\centering  
%\subfigure[3D view.]{\centering \includegraphics[width=\columnwidth]{img/Ex1_3D.eps}\label{fig:ex1_3d}}
%\qquad
%\subfigure[XZ view in $\mathcal{R}^{+}$.]{\centering \includegraphics[width=0.48\columnwidth]{img/Ex1_2D_left.eps}\label{fig:ex1_xy_l}}
%\vspace{0.1mm}
%\subfigure[XZ view in $\mathcal{R}^{-}$.]{\centering \includegraphics[width=0.48\columnwidth]{img/Ex1_2D_right.eps}\label{fig:ex1_xy_r}}
%\caption{Results of the end-effector collision avoidance experiment.}
%\label{fig:exp_1}
%\end{figure}
%
%
%\begin{figure*}[!t]
%\centering  
%\subfigure[Original trajectory starting at $\bfx_{1}(0) = {[}-0.52, 0.5, 0.02 {]}^{T} \in \mathcal{R}^{+}$.]{\centering \includegraphics[width=\columnwidth]{img/Snapshot_Ex1_left_c.png}\label{fig:ex1_snap_l_c}}
%\vspace{0.1mm}
%\subfigure[Original trajectory starting at $\bfx_{1}(0) = {[}-0.52, -0.5, 0.02 {]}^{T} \in \mathcal{R}^{-}$.]{\centering \includegraphics[width=\columnwidth]{img/Snapshot_Ex1_right_c.png}\label{fig:ex1_snap_r_c}}
%\qquad
%\subfigure[Reshaped trajectory starting at $\bfx_{1}(0) = {[}-0.52, 0.5, 0.02 {]}^{T} \in \mathcal{R}^{+}$.]{\centering \includegraphics[width=\columnwidth]{img/Snapshot_Ex1_left.png}\label{fig:ex1_snap_l}}
%\vspace{0.1mm}
%\centering
%\subfigure[Reshaped trajectory starting at $\bfx_{1}(0) = {[}-0.52, -0.5, 0.02 {]}^{T} \in \mathcal{R}^{-}$.]{\centering \includegraphics[width=\columnwidth]{img/Snapshot_Ex1_right.png}\label{fig:ex1_snap_r}}
%\qquad
%\caption{Snapshots of the end-effector collision avoidance task execution for different starting positions.}
%\label{fig:snap_exp_1}
%\end{figure*}
%
%\subsubsection{Joint Space Collision Avoidance}
%This experiment shows the scalability of the proposed approach in high dimensional spaces and its ability to reshape high order DS. The task is a point-to-point motion in the joint space from $\bfx_{1}(0) = [35, 55, 15, -65, -15, 50, 90]^T ~deg$ to $\hat{\bfx}_1 = [-60, 30, 30, -70, -15, 85, 15]^T ~deg$. The original joint position trajectory is obtained by numerically integrating ($\delta t = 0.005~s$) the second-order DS
%\begin{equation}
%\label{eq:joint_ds}
%	\begin{split}
%		\dot{\bfx}_1 &= \bfx_2\\
%		\dot{\bfx}_2 &= 2(\hat{\bfx}_1 - \bfx_1) - 2\sqrt{2}\bfx_2
%	\end{split}
%\end{equation} 
%where $\bfx_1 = [\theta_1,\ldots,\theta_7]^T \in \mathbb{R}^7$ are the joint angles and $\bfx_2 \in \mathbb{R}^7$ the joint velocities. The system (\ref{eq:joint_ds}) has a GAS equilibrium at $\hat{\bfx} = [\hat{\bfx}_1^T \mathbf{0}^T]^T \in \mathbb{R}^{14}$ and Lyapunov function $V = \frac{1}{2}(\hat{\bfx}_1 - \bfx_1)^{T}(\hat{\bfx}_1 - \bfx_1) + \frac{1}{2}\bfx_{2}^{T}\bfx_2$. The original joint angles trajectories are shown in Fig. \ref{fig:exp_2} (black solid lines).
%
%As shown in Fig. \ref{fig:overview}, following the original trajectory the robot hits an unforeseen obstacle (the red bar in Fig. \ref{fig:overview}). A kinesthetic demonstration is then provided (red lines in Fig. \ref{fig:exp_2}) to avoid the collision. With the reshaped trajectory (blue lines in Fig. \ref{fig:exp_2}) the robot is able to avoid the obstacle (Fig. \ref{fig:overview}) and to reach the desired goal $\hat{\bfx}_1$. Results are obtained with noise variance $\sigma_{n}^{2} = 0.1$, signal variance $\sigma_{k}^{2} = 1$, length scale $l=0.01$ and the threshold $\bar{c} = 15 ~deg$. With the adopted $\bar{c}$ only $27$ points over $178$ are added to the GP. 
%
%\begin{figure}[!htb]
%\centering  
%\includegraphics[width=\columnwidth]{img/Ex2.eps}
%\caption{Original joint angles trajectories (black lines), the provided demonstration (red lines) and reshaped joint angles trajectories (blue lines) for the joint space collision avoidance experiment.}
%\label{fig:exp_2}
%\end{figure}
%%\begin{itemize}
%%	\item \textcolor{red}{Not working because joint do not reach the goal}
%%\end{itemize}
%
%\subsection{Discussion}
%%Results presented in this section underline notable characteristics of the proposed approach, that are:
%%\begin{itemize}
%%\item Incremental learning of novel behaviours. 
%%\item Learning of multi-modal behaviours. 
%%\item Reshaping of high-order, non-linear DS without affecting their stability.
%%\item Scalability in high dimensional spaces.
%%\end{itemize}
%The proposed approach works for DS of any order, as underlined in Sec. \ref{sec:DS_Modulation}. Nevertheless, being robot manipulators dynamics described by second-order DS, a second-order DS is sufficient to generate dynamically feasible trajectories. For this reason, we show results for DS up to the second order.
%
%The adopted control law in (\ref{eq:u_param}) pushes the robot position towards the demonstrated position, without considering desired velocities or accelerations. We adopt this solution because, in the majority of the cases, a user is interested in reconfiguring the robot and he can hardly show a desired velocity (or acceleration) behaviour through kinesthetic teaching.
%
%It must be noted that the proposed control law (\ref{eq:u_param}) does not always guarantee good tracking of the demonstrated trajectories, as shown in Fig. \ref{fig:exp_2}. In general, to have good tracking performance, different controllers have to be designed for different DS \cite{Slotine91}. Nevertheless, we are not interested in accurately track the demonstrated trajectories, but we want to modify the robot's behaviour until the task is correctly executed. The joint angle trajectories in Fig. \ref{fig:exp_2} guarantee the correct execution of the task, i.e. the robot converges to the desired joint position while avoiding the obstacle.      
%
%Having a pure elastic forcing term as in (\ref{eq:u_param}) can generate overshoots in the resulting position trajectory, as shown in Fig. \ref{fig:exp_2} (see the angle $\theta_6$). The overshoot problem can be alleviated, in principle, by adding to (\ref{eq:u_param}) a damping term depending on the velocity. In this work, we do not adopt such a strategy for three reasons. First, adding a damping term does not guarantee to avoid overshoots for any kind of DS. Second, adding a damping term means increasing the parameter space. Third, as already mentioned, our goal is not to exactly track the demonstrated data.      
